Nearly-optimal Robust Matrix Completion

In this paper, we consider the problem of Robust Matrix Completion (RMC) where the goal is to recover a low-rank matrix by observing a small number of its entries out of which a few can be arbitrarily corrupted. We propose a simple projected gradient descent method to estimate the low-rank matrix that alternately performs a projected gradient descent step and cleans up a few of the corrupted entries using hard-thresholding. Our algorithm solves RMC using nearly optimal number of observations as well as nearly optimal number of corruptions. Our result also implies significant improvement over the existing time complexity bounds for the low-rank matrix completion problem. Finally, an application of our result to the robust PCA problem (low-rank+sparse matrix separation) leads to nearly linear time (in matrix dimensions) algorithm for the same; existing state-of-the-art methods require quadratic time. Our empirical results corroborate our theoretical results and show that even for moderate sized problems, our method for robust PCA is an an order of magnitude faster than the existing methods.

==> conc.tex <==
\section{Conclusion}
In this work, we studied the Robust Matrix Completion problem. For this problem, we provide exact recovery of the low-rank matrix $\Lo$ using nearly optimal number of observations as well as nearly optimal fraction of corruptions in the observed entries. Our RMC result is based on a simple and efficient PGD algorithm that has nearly linear time complexity as well. Our result improves state-of-the-art for the related Matrix Completion as well as Robust PCA problem. For Robust PCA, we provide first nearly linear time algorithm under standard assumptions. 

Our sample complexity depends on $\epsilon$, the desired accuracy in $\Lo$. We believe that the arguments used by \cite{}, we should be able to remove the $\epsilon$ dependence as well and leave it for future work. Moreover, improving dependence of sample complexity on $r$ (from $r^2$ to $r$) also represents an important direction. Finally, similar to foreground background separation, we would like to explore more applications of RMC/RPCA. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

